Personalized Security Indicators to Detect Application Phishing Attacks in Mobile Platforms

Phishing in mobile applications is a relevant threat with successful attacks reported in the wild. In such attacks, malicious mobile applications masquerade as legitimate ones to steal user credentials. In this paper we categorize application phishing attacks in mobile platforms and possible countermeasures. We show that personalized security indicators can help users to detect phishing attacks and have very little deployment cost. Personalized security indicators, however, rely on the user alertness to detect phishing attacks. Previous work in the context of website phishing has shown that users tend to ignore the absence of security indicators and fall victim of the attacker. Consequently, the research community has deemed personalized security indicators as an ineffective phishing detection mechanism. We evaluate personalized security indicators as a phishing detection solution in the context of mobile applications. We conducted a large-scale user study where a significant amount of participants that used personalized security indicators were able to detect phishing. All participants that did not use indicators could not detect the attack and entered their credentials to a phishing application. We found the difference in the attack detection ratio to be statistically significant. Personalized security indicators can, therefore, help phishing detection in mobile applications and their reputation as an anti-phishing mechanism should be reconsidered. We also propose a novel protocol to setup personalized security indicators under a strong adversarial model and provide details on its performance and usability.

==> detection.tex <==

\section{Improved Centralised Detection}
\label{sec:centralised}

In this section we describe two ways to address the limitations of centralised phishing detection identified in Section~\ref{sec:comparison}.


\subsection{Directory of Sideloaded Applications}

The mobile platform application installer can be modified to upload every sideloaded third-party application to the central application marketplace for analysis. The marketplace can perform two types of analysis. First, the name of the sideloaded application can be compared to other applications in the marketplace. If applications with a similar name are found, the marketplace can send a warning message back to the application installer that notifies the user. Based on this information, the user may choose to abort or continue with the installation (i.e., the installation decision does not need to be conditional to approval of the centralised authority, but rather a choice of the user).

Second, the marketplace operator can, at a later point in time, manually inspect all sideloaded applications that have a name similar to applications already existing in the marketplace database. Information about any application that is found malicious by such offline analysis, can be communicated back to installer that may suggest to the user the removal of the installed phishing application. Android already implements such \emph{killswicth} functionality. This simple application installer modification turns the application marketplace into a \emph{name directory} of all Android applications, both centrally published and sideloaded. 

This approach provides the security benefits of a closed system, namely centralised malware detection, while retaining the functionality of an open application platforms, namely ability for developers to distribute their applications without approval from a single authority. The drawback is that such phishing application detection would have both false negatives and false positives. 

To estimate the number of false positives, we examined a data set of application names from Android marketplace (\red{add reference}). The data set contained (\red{xx}) names downloaded from the Android marketplace in 2011. The data set contained (\red{xx}) applications with exactly the same name, (\red{xx}) applications with single character difference in the name, and (\red{xx}) applications with a two-character difference in the name. The numbers imply that... (\red{add some BS reasoning}) 

While repeated false warnings are well known to cause user habituation to ignore all security warnings (\red{add reference}), this approach would provide an easily deployable detection scheme for similarity attacks.


\subsection{Visual Similarity Detection}

In background and forwarding attacks the name of the application may be different, but the phishing application user interface changes to match the target application UI. Detection of background and forwarding attacks could be addressed by detecting user interface similarity of mobile applications. 

User interface similarity detection for phishing protection has been studied in the context of web sites \cite{chen10tit} (\red{more references}). In a typical web site similarity detection scheme, the web page DOM tree is parsed, textual and image elements are compared. Similar detection schemes could be adapted for mobile applications. User interfaces of Android applications are typically defined in XML configuration files, although user interfaces can be defined and modified in Java code as well. A simple mobile application user interface similarity detection mechanism could search for similarities in XML configurations files. A more sophisticated detection scheme could attempt to detect similar user interface constructs at Java-code level. We are not aware or any prior work on mobile application Visual similarity detection and consider this an interesting direction for further work.

Visual similarity detection would provide the typical strengths of any centralised detection scheme: no user effort and no limitations on existing mobile platform functionality. The drawbacks are well known from any malware detection scheme: benign applications have significant similarities in their user interfaces (false positives) and the adversary could find alternative ways to construct similar user interfaces depending on the chosen detection heuristic (false negatives). 


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 


==> discussion.tex <==

\section{Discussion}
\label{sec:discussion}

Our goal is to provide the \emph{technical means} to configure application indicators securely.
In the following we briefly discuss important aspects of our solution,
including what is the best type of personal indicator, or how effective application indicators are in the context of applications phishing attacks.
However, we set a thorough study of these issues as future work.


\subsection{Security Indicator Type}

Various types of application indicators have been proposed by previous research; pass-phrases and pictures are common examples~\cite{tygar96woec}.
A mobile application can show a pass-phrase or a picture indicator on a dedicated area of the application GUI; alternatively, the picture
can be used as the background image of the application~\cite{dhamija05soups}.

The authentication scheme that uses the application indicator can be either \emph{passive} or \emph{interactive}.
In a passive scheme, the user implicitly checks the correctness of the displayed application indicator.
In an interactive, or conditioned scheme, the user must explicitly acknowledge the presence of the correct security indicator \cite{herzberg12, karlof09ndss}.
For example, the application might force the user to select the correct picture from a small set of candidate pictures, before he can start using the application.
Interactive schemes increase the required user effort, but provide better phishing detection~\cite{herzberg11esorics, karlof09ndss}.

The application indicator can either be shown to the user only when the application is started, or it can be continuously displayed while the application is active.
Showing the application indicator at startup is sufficient to address similarity attacks.
Continuous indicators are needed to protect from  background and forwarding attacks.
The drawback of continuous indicators is that a part the mobile application GUI has to be persistently reserved for the indicator.
This can be a problem in mobile applications with limited screen area.

Ultimately, the choice of the application indicator type depends on the scenario.
Applications providers with high security requirements (e.g., banks) can adopt indicators with good security properties (e.g., interactive verification and continuous display).
Other providers can choose indicators that require less user effort and impose fewer restrictions on GUI design (e.g., passive verification at startup).


\subsection{Security Indicator Effectiveness}

The effectiveness of security indicators has been studied primarily in the context of websites.
While prior studies have shown that users tend to ignore them~\cite{schechter07sp,lee-w2sp14},
more recent experiments suggest that visual security indicators can be effective when correctly designed and deployed~\cite{herzberg11esorics, herzberg12, akhawe13usenix}.
Interactive indicators typically exhibit higher phishing detection rates~\cite{akhawe13usenix, karlof09ndss, herzberg11esorics, radke-ozhci13}.
A recent study on effectiveness of security indicators for \emph{mobile browsers} shows that the small screen of a mobile device can make security indicators less effective~\cite{amrutkar-mobcomp13}.
As expected, user training improves detection of web phishing attacks~\cite{kumaraguru-ecrime07, kumaraguru-soups09}.

Besides mobile browsers, we are not aware of any previous user study on the effectiveness of application indicators in mobile platforms.
In contrast to a general-purpose mobile application (e.g., a browser), a dedicated mobile application (e.g., a banking application) can potentially allocate a significant part
of its user interface for the indicator.
User studies on effectiveness of different indicators types for mobile applications is a natural direction for future work.
Also the ability of the user to start and complete the setup protocol must be evaluated.


\subsection{Deployment Aspects}

The protocol described in Section~\ref{sec:appid-setup} requires the application provider to setup an online server.
Given that a large number of applications communicate with the infrastructure of their providers (to consolidate user rankings, to store user's profiles, etc.), we argue that
the needed infrastructure already exists for many application scenarios. For mobile application providers that do not run online servers, the cost of adopting our solution is naturally higher.
From the results of our evaluation (see Section~\ref{sec:appid-setup}), we conclude that the setup of an application indicator is inexpensive in terms of computation and communication;
hence, the solution can easily scale for services with a large number of users.

The setup mechanism requires an out-of-band (OOB) communication between the application provider and the user.
Examples of OOB channels include postal mail, web or email communication via a trusted device like a PC.
The mobile platform itself cannot be used as the OOB channel because a malicious application could inject fabricated messages, for example, by mounting a background attack.
The indicator setup mechanism can easily be adopted by application providers that already have established OOB channels to users (e.g., banks regularly send letters to their customers).

Our implementation requires the provider to send a service tag along with the
PIN in order for the \secmodule{} to measure the correct application.
This design choice increases the amount of data that the user has to type into the \secmodule{} (10 characters in the prototype implementation).
The length of the user input can be reduced, e.g., by allowing the user to select the target application by other means (e.g., the \secmodule{} could present a list of applications for the user to choose).


%\subsection{Future Work}
%
%Detection of phishing applications based on visual similarity is an additional direction for future work. Phishing detection based on visual similarity has been studied in the context of websites~\cite{chen10tit, maurer-css12}. We are not aware of any previous work on phishing detection of visually similar mobile applications... Formalise active applications transitions on a mobile system and evaluate possible attacks... TrustZone prototype of the solution...



%Another important usability issue is the design of the personalized security
%indicator. Existing security indicator designs include proposals that need only
%user attention, for example, focusing on coloured address
%bars~\cite{almuhimedi-soups08}, customized GUI~\cite{dhamija05soups}, etc. There
%are also several solutions that require active user participation; examples of
%this approach include picking the correct indicator from a set~\cite{herzberg12}
%or using an SAS~\cite{wu-soups06}.

%Our solution requires active user
%participation during application installation and execution. At install time,
%the user should adhere to the broker-facilitated setup instructions such as the
%use of the secure-attention-sequence (SAS) and finally, check the
%authentication-tag to verify the successful installation of the correct
%application. During the use of the application itself, the user must
%continuously track his personalized application indicator to ensure that he is
%talking to the correct application. This increased burden on the user also
%implies that our solution is best suited for sensitive applications (like mobile
%banking) that warrant such a high degree of security against phishing attacks.

%Moreover, it has been shown that
%training~\cite{kumaraguru-ecrime07, kumaraguru-soups09} improves a user's
%ability to detect web phishing attacks. Therefore, it would be interesting to
%investigate ways (e.g., user training, better design of indicators) to improve
%the effectiveness of our solution.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

